Fast And Automatic Floating Point Error Analysis With CHEF-FP

As we reach the limit of Moore's Law, researchers are exploring different paradigms to achieve unprecedented performance. Approximate Computing (AC), which relies on the ability of applications to tolerate some error in the results to trade-off accuracy for performance, has shown significant promise. Despite the success of AC in domains such as Machine Learning, its acceptance in High-Performance Computing (HPC) is limited due to stringent requirements for accuracy. We need tools and techniques to identify regions of code that are amenable to approximations and their impact on the application output quality to guide developers to employ selective approximation. To this end, we propose CHEF-FP, a flexible, scalable, and easy-to-use source-code transformation tool based on Automatic Differentiation (AD) for analyzing approximation errors in HPC applications. CHEF-FP uses Clad, an efficient AD tool built as a plugin to the Clang compiler and based on the LLVM compiler infrastructure, as a backend and utilizes its AD abilities to evaluate approximation errors in C++ code. CHEF-FP works at the source by injecting error estimation code into the generated adjoints. This enables the error-estimation code to undergo compiler optimizations resulting in improved analysis time and reduced memory usage. We also provide theoretical and architectural augmentations to source code transformation-based AD tools to perform FP error analysis. This paper primarily focuses on analyzing errors introduced by mixed-precision AC techniques. We also show the applicability of our tool in estimating other kinds of errors by evaluating our tool on codes that use approximate functions. Moreover, we demonstrate the speedups CHEF-FP achieved during analysis time compared to the existing state-of-the-art tool due to its ability to generate and insert approximation error estimate code directly into the derivative source.

==> backup/background.tex <==
\section{Background}

Most real-valued applications heavily rely on FP arithmetic. However, due to the finite nature of computing, it is incredibly hard to exactly represent a lot of the real values as FP numbers. This inexactness inevitably leads to errors that can grow quickly and have serious implications on the accuracy of the application. These errors born out of squeezing the infinite real-valued numbers into a finite set of bits are known as \emph{rounding errors}.

The FP rounding error is accumulated contribution of FP errors from each variable to the target function's result. These target functions are modeled as a series of multiple assignment operations, we assume that these assignments and inputs to the functions are independent (FP error analysis on correlated variables is still a nascent field and definitive methods of estimation are yet to be established). For each such assignment we then define an expression that calculates and accumulates the FP error introduced by that assignment. We refer to these error calculation and accumulation expressions as FP error models. Our tool, with it's default error model, aims to estimate an upper bound on these FP rounding errors. 

\subsection{Modelling FP Errors}
\label{sec:fpmodel}

The error model describes a metric which can be used in error estimation analysis. This metric is applied to all assignment operations in the function and the results from the evaluation of the metric are accumulated into the total FP error contributed by the left-hand side of the assignment. The Taylor series approximation is well fit to model floating point errors. Let's assume an arbitrary function \(y = f(x)\), where \(x\) is represented in the standard IEEE 754 single precision. Assuming a floating point error of \(h\) in \(x\), we define \(\widetilde{f}(x) = f(x + h) \). A symbolic Taylor series expansion yields the following:
\[ f(x + h) = f(x) + \frac{h}{1!}f'(x) + \frac{h^2}{2!}f''(x) + \frac{h^3}{3!}f'''(x) + ...
\]

Here \(f'(x)\) represents the derivative of the function with respect to \(x\). Approximating the series to its first order results in the following:
\[ f(x + h) = f(x) + \frac{h}{1!}f'(x) + O(h^2)
\]

An expression for the absolute floating point error in \(f\) can be represented as:
\[ A_f = | \widetilde{f}(x) - f(x) |
   => A_f = | \frac{h}{1!}f'(x) | 
   => A_f = | hf'(x) |
\]

To determine the maximum absolute floating point error in \(f\) we write \(h = \epsilon_m |x|\) where \(\epsilon_m\) is known as the \textit{machine epsilon}. The machine epsilon gives the maximum relative representation error in floating point variables due to rounding. It is a machine dependant value and follows the IEEE standard in most compilers. The absolute error can be written as:
\begin{equation}
 \label{eqn:deftmodel}    
 A_f=|\epsilon_m|x|f'(x)|
\end{equation}

This default model is sufficient for most smaller cases and can produce loose upper bounds of the maximum permissible FP error in programs. %\mynote{Expand.}
%FIXME: Move to implementation details;We provide a simple class interface that users can implement to develop their error models. We also provide comprehensive demos on how to code up a custom error model from scratch.

The computational efficiency of the Taylor-based approximations can be achieved using techniques available in automatic differentiation.

\subsection{Automatic Differentiation Basics}

%Automatic differentiation uses the properties of the chain rule to evaluate differential operators of a function that is represented as a computer program. A differential operator maps an input function to a new function that captures how small perturbations in the inputs affect the output. First-order differential operators of real-valued functions include directional derivatives and gradients~\cite{betancourt2018geometric}. A differential operator, or a \textit{pushforward}, maps between the local tangent space of the input (the space of perturbations to the inputs) to the local tangent space of the outputs. Informally, a pushforward takes a wiggle in the input space, and tells what wobble is created in the output space, by passing it through the function. The \textit{pullback} operator maps the cotangent space of the outputs to the inputs. Informally, the pullback takes wiggles with respect to the function’s output, and tells the equivalent wobble with respect to the functions input.

AD takes as input program code that \textit{has meaningful differentiable properties} and produces new code augmented with pushforward or pullback operators. The AD mode which produces pushforward operators to capture the sensitivity from inputs to outputs is commonly known as \textit{forward} mode. The AD mode capturing the sensitivity from outputs to inputs is called \textit{reverse} mode, \textit{adjoint} mode, or backpropagation in ML. The mathematical and computational merit of the pullback is that it provides an extremely eﬀicient way to compute the gradient of a function with relative time complexity which is independent of the input size~\cite{griewank2008evaluating}.

AD tools can be categorized by how much work is done before program execution. AD typically starts by \textit{building a computational graph}, or a directed acyclic graph of mathematical operations applied to an input. At one extreme, the \textit{tracing}, or \textit{taping}, approach constructs and processes the computational graph at the time of execution, each time a function is invoked. In contrast, the source transformation approach does as much as possible at compile time to create the derivative only once. The tracing approach is easier to implement and adopt into existing codebases. The source transformation approach has better performance, but usually covers a subset of the language.
\textbf{Tracing:} Records the linear sequence of
computation operations at runtime into a \textit{tape} (or Wengert list~\cite{wengert1964simple}). The control flow is flattened to produce a derivative. A typical implementation is via operator overloading, defining a special floating type with overloaded elementary  operations. Algorithms use this type to trigger   differentiation by calling a special function. There are numerous C++ AD tools  based on tracing including ADOL-C~\cite{griewank1996algorithm}, CppAD~\cite{bell2011cppad}, and Adept~\cite{hogan2014fast}. As the derivative is produced at runtime, the just-in-time differentiation process is constrained to perform optimizations quickly.
Metaprogramming techniques, such as expression templates, can mitigate the issue but they cannot optimize across  statements and generally do not handle control flow~\cite{hogan2014fast, JonesVarid, sagebaum2018expression}.
\textbf{Source Transformation:} Constructs  the computation graph and produces a derivative function at compile time. More compiler optimizations can be applied, such as reorganizing or evaluating simple constant expressions at compile time and common subexpression elimination. Source transformation is more difficult to  implement as it requires a significant investment in developing and maintaining a language parser. Tapenade~\cite{hascoet2013tapenade} is an example for a source transformation tool with custom parsers for C and Fortran. Source transformation tools usually do not support the full feature set of a language (e.g. certain language idioms are particularly hard to differentiate).

Historically, toolmakers made trade offs between ease of use, performance and ease to integration. AD now benefits from better language support to avoid such trade offs. Recently, production compilers like Clang allowed tools to reuse the language parsing infrastructure. Enzyme~\cite{enzymeNeurips} and Clad~\cite{clad} are compiler-based AD tools using source transformation.

\subsection{FP Error Sensitivity Analysis}

An important aspect of dealing with FP applications with high precision requirements is realizing the sensitive, or more error-prone, areas to devise suitable mitigation strategy. This is where AD-based sensitivity analysis can be very useful. It can help determine specific variables or regions of code that have a higher contribution to the overall FP error in the application. 

The sensitivity of a variable \(x\) to FP errors (\(S_x\)) can be deduced from the default error model described in Eq. \ref{eqn:deftmodel} as:
\[S_x = | x f'(x) |\]

Here, the total contribution of FP errors to the function by variable \(x\) increases as \(S_x\) increases. A study of the trends of these sensitivity values across the domain of a function can reveal interesting insights into the numerical stability of the function and can also help determine possible causes of these instabilities. These sensitivity values can also be used as a guide for a class of type-based optimizations called \emph{Mixed Precision Tuning}.  

\subsection{Mixed Precision Tuning}

It is considered a safe practice to implement applications with high precision requirements in the highest precision available (such as the 10-byte extended precision format - long double) on the machine. These high precision configurations often entail a higher execution time and more memory consumption. Moreover, for a lot of HPC applications on accelerated hardware such as the current generation GPUs, higher precision comes at a much higher cost (if at all it is even available). This motivates the analysis of applications to find mixed precision configurations that have an agreeable difference in the final accuracy of the application. Mixed Precision Tuning is one way to perform such optimizations.

Mixed Precision Tuning involves \textit{demoting} certain variables to lower precision in an application without severely affecting the overall accuracy of the application. In corollary, it involves preserving or \textit{promoting} the precision of variables that have a significant affect on the accuracy of the application. A mixed precision tuned configuration is only valid when the difference the pre- and post tuning accuracy is less than some user set threshold value. An effective way to maintain this requirement is analysing the sensitivity of all input and intermediate variables in the application and selecting the ones with lower sensitivity to be demoted. The FP error contributions of all these demoted variables are accumulated and then compared to the threshold value. A mixed precision configuration is reached when the accumulated error satisfies the threshold value.


While many AD based approaches exist for error-analysis, they typically involve significant manual effort to perform code changes or long toolchain to automate it. In this work, we present an AD based FP error estimation framework that requires little to no manual integration work, and comes packaged with the AD backend Clad, taking away the tedious task of setting up long tool chains. The tool's proximity to the compiler and the fact that the FP error annotations are built into the code's derivatives allows for powerful compiler optimizations that provide significant speedups of the analysis time when compared to the current state-of-the-art tools like ADAPT~\cite{menon2018adapt}.

==> backup/introduction.tex <==
\section {Introduction}
\label{sec:introduction}
%\mynote{Garima: Profile why we take less memory and if that's the case put that as a statement here.}
Floating-point arithmetic operations are the most prevalent computation
in HPC applications. Computer architectures support multiple levels of
precision for floating-point (FP) data and arithmetic operations. In the IEEE 754 standard, the
most common representation today for real numbers, choices are 64 bits \emph{double} precision,
32 bits \emph{single} precision, 128 bits \emph{quad} precision, and 16 bits \emph{half} precision. The choice
of precision determines the amount of rounding error. 
Therefore, we need to be prudent about how and where lower-precision computing is
applied in a HPC code.
While using higher precision for data and operations may result in increased accuracy, it can lead
to an increase in application execution time, memory and energy consumption. Hence, we want
to use higher precision when necessary to maintain accuracy and use lower precision where
we can improve performance.
Despite the availability of multiple levels of precision for floating-point, it is 
challenging to apply them in HPC and scientific codes. However, to use them effectively,
developers need to understand the details of floating-point rounding errors as well as 
how they propagate through their application.
Due to the lack of scalable and rigorous tools that analyse
error sensitivity in the applications’ code regions, developers often
resort to the safer option of using high precision (\emph{double}) throughout the code. 
We need scalable tools to understand the impact of lowering the precision of 
data and computation, identify error tolerant code regions, and provide guidance to the users.

Several techniques have been proposed to estimate the sensitivity profile of an application,
including automated search based approaches~\cite{rubio2013precimonious,lam2018fine}, static analysis~\cite{das2021robustness}, or using AD~\cite{menon2018adapt}.
Unfortunately, the existing set of tools fail to provide a feasible solution for HPC applications. 
The search-based approaches evaluate different mixed-precision configurations to identify a
configuration that satisfies a given error threshold. This is a very expensive process as the
state space is significantly large (exponential in the number of variables or operations) and
quickly becomes infeasible even for a small benchmark. Static analysis based approaches using
interval analysis or Taylor series approximation provide rigorous estimate for FP
errors. However, they are not scalable and are limited to programs with a small number of operations. 
Several methods~\cite{menon2018adapt} leverage AD to determine error resilient regions of the code have been
proposed. While they have been shown to work well for smaller HPC benchmarks, they often require
manual code changes and incorporates several software tools in a toolchain~\cite{lam2019floatsmith}.  
These tools have high memory overhead and are slow, making it infeasible for large HPC workloads.


% Stuff added by Garima 

% Our contribution builds on the work by Harshitha Menon et al. on ADAPT. ADAPT is a floating-point (FP) error estimation tool that efficiently delivers mixed-precision configurations for C++ codes using operator overloading based automatic differentiation (AD). While ADAPT's approach is succinct and practical for smaller workloads,  it exposes a set of points for optimization and automatization on larger projects. 

We use Clad~\cite{clad}, an efficient AD tool built as a plugin to the Clang compiler and based on the LLVM compiler infrastructure. We use Clad as a backend for the presented framework and utilize its AD abilities to evaluate floating-point errors in C++ code. Clad implements source code transformation based AD, i.e., it inspects the internal compiler representation of a program to generate its derivative. This level of granularity allows Clad to exploit a program's source information to automatically add auxiliary instructions to the generated gradient depending on a set of rules. Accordingly, we can annotate code with floating point error information without user intervention. This automation is beneficial for large-scale codes wherein going in to hand-write annotations becomes complex, tedious and error-prone.

Moreover, we enable the possibility of domain specific FP error analysis due to the increased flexibility of a compiler-based backend. This allows easy modification of parts of the framework to achieve a more tailored FP error analysis. This level of variability also enables a  finer-grained analysis where users can themselves query source information and make more precise decisions for the direction of the analysis.     

Finally, because we generate FP error estimation (EE) code directly into the derivative source, we observe a significant speedup compared to other tools performing similar FP error analysis. The generated code also becomes a candidate for further compiler optimizations contributing to better runtime performance overhead.
We use the FP error profile provided by our tool to guide the design of mixed-precision version of the code and achieve significant performance improvements while satisfying the user-specified error threshold.

% \mynote{Compare with existing works and highlight their shortcomings.}

% \mynote{Add a list of contributions.}
\textbf{Key Contributions}
\begin{itemize}
    \item An efficient tool to automate AD-based FP error analysis. The output of the tool guides developers to design a mixed-precision version of code;
    \item Formalism defining augmenting the AD transformation to aid FP error analysis;
    \item Customizable EE module that supports any AD-based user defined error model.
    \item Tool evaluation using a set of HPC benchmarks for mixed-precision and approximate function error analysis.
\end{itemize}

==> coverLetter.tex <==
Cover Letter
